Joint Waveform and Passive Beamformer Design in Multi-IRS-Aided Radar

Intelligent reflecting surface (IRS) technology has recently attracted a significant interest in non-light-of-sight radar remote sensing. Prior works have largely focused on designing single IRS beamformers for this problem. For the first time in the literature, this paper considers multi-IRS-aided multiple-input multiple-output (MIMO) radar and jointly designs the transmit unimodular waveforms and optimal IRS beamformers. To this end, we derive the Cramer-Rao lower bound (CRLB) of target direction-of-arrival (DoA) as a performance metric. Unimodular transmit sequences are the preferred waveforms from a hardware perspective. We show that, through suitable transformations, the joint design problem can be reformulated as two unimodular quadratic programs (UQP). To deal with the NP-hard nature of both UQPs, we propose unimodular waveform and beamforming design for multi-IRS radar (UBeR) algorithm that takes advantage of the low-cost power method-like iterations. Numerical experiments illustrate that the MIMO waveforms and phase shifts obtained from our UBeR algorithm are effective in improving the CRLB of DoA estimation.

==> ICASSP 2023_ Joint Waveform and Beamforming Design in Multi-IRS Aided Radar/symbols.tex <==
%% Short symbol commands for LaTex
\usepackage{amsmath}
%\usepackage{algpseudocode}
\usepackage{amsthm}
\usepackage{dsfont}
%\usepackage{algorithm}
%\usepackage[lined,boxed,commentsnumbered]{algorithm2e}
\usepackage{thmtools}
\usepackage{amssymb}
\usepackage[dvipsnames]{xcolor}
\def \Version{2.0.10}
\def \Update{\today}

% Lower case bold English alphabets
\def\ba{\boldsymbol{a}}
\def\bb{\boldsymbol{b}}
\def\bc{\boldsymbol{c}}
\def\bd{\boldsymbol{d}}
\def\be{\boldsymbol{e}}
\def\bdf{\boldsymbol{f}}
\def\bg{\boldsymbol{g}}
\def\bh{\boldsymbol{h}}
\def\bi{\boldsymbol{i}}
\def\bj{\boldsymbol{j}}
\def\bk{\boldsymbol{k}}
\def\bl{\boldsymbol{l}}
\def\bm{\boldsymbol{m}}
\def\bn{\boldsymbol{n}}
\def\bo{\boldsymbol{o}}
\def\bp{\boldsymbol{p}}
\def\bq{\boldsymbol{q}}
\def\br{\boldsymbol{r}}
\def\bs{\boldsymbol{s}}
\def\bt{\boldsymbol{t}}
\def\bu{\boldsymbol{u}}
\def\bv{\boldsymbol{v}}
\def\bw{\boldsymbol{w}}
\def\bx{\boldsymbol{x}}
\def\by{\boldsymbol{y}}
\def\bz{\boldsymbol{z}}

% Upper case bold English alphabets
\def\bA{\boldsymbol{A}}
\def\bB{\boldsymbol{B}}
\def\bC{\boldsymbol{C}}
\def\bD{\boldsymbol{D}}
\def\bE{\boldsymbol{E}}
\def\bF{\boldsymbol{F}}
\def\bG{\boldsymbol{G}}
\def\bH{\boldsymbol{H}}
\def\bI{\boldsymbol{I}}
\def\bJ{\boldsymbol{J}}
\def\bK{\boldsymbol{K}}
\def\bL{\boldsymbol{L}}
\def\bN{\boldsymbol{N}}
\def\bM{\boldsymbol{M}}
\def\bO{\boldsymbol{O}}
\def\bP{\boldsymbol{P}}
\def\bQ{\boldsymbol{Q}}
\def\bR{\boldsymbol{R}}
\def\bS{\boldsymbol{S}}
\def\bT{\boldsymbol{T}}
\def\bU{\boldsymbol{U}}
\def\bV{\boldsymbol{V}}
\def\bW{\boldsymbol{W}}
\def\bX{\boldsymbol{X}}
\def\bY{\boldsymbol{Y}}
\def\bZ{\boldsymbol{Z}}

% Bold Greek alphabets
\def\balpha{\boldsymbol{\alpha}}
\def\bbeta{\boldsymbol{\beta}}
\def\bgamma{\boldsymbol{\gamma}}
\def\bGamma{\boldsymbol{\Gamma}}
\def\bdelta{\boldsymbol{\delta}}
\def\bDelta{\boldsymbol{\Delta}}
\def\bepsilon{\boldsymbol{\epsilon}}
\def\bvarepsilon{\boldsymbol{\varepsilon}}
\def\bzeta{\boldsymbol{\zeta}}
\def\bdeta{\boldsymbol{\eta}}
\def\btheta{\boldsymbol{\theta}}
\def\bvartheta{\boldsymbol{\vartheta}}
\def\bTheta{\boldsymbol{\Theta}}
\def\biota{\boldsymbol{\iota}}
\def\bkappa{\boldsymbol{\kappa}}
\def\blambda{\boldsymbol{\lambda}}
\def\bLambda{\boldsymbol{\Lambda}}
\def\bmu{\boldsymbol{\mu}}
\def\bnu{\boldsymbol{\nu}}
\def\bxi{\boldsymbol{\xi}}
\def\bXi{\boldsymbol{\Xi}}
\def\bpi{\boldsymbol{\pi}}
\def\bPi{\boldsymbol{\Pi}}
\def\brho{\boldsymbol{\rho}}
\def\bvarrho{\boldsymbol{\varrho}}
\def\bsigma{\boldsymbol{\sigma}}
\def\bSigma{\boldsymbol{\Sigma}}
\def\btau{\boldsymbol{\tau}}
\def\bupsilon{\boldsymbol{\upsilon}}
\def\bUpsilon{\boldsymbol{\Upsilon}}
\def\bphi{\boldsymbol{\phi}}
\def\bvarphi{\boldsymbol{\varphi}}
\def\bPhi{\boldsymbol{\Phi}}
\def\bchi{\boldsymbol{\chi}}
\def\bpsi{\boldsymbol{\psi}}
\def\bPsi{\boldsymbol{\Psi}}
\def\bomega{\boldsymbol{\omega}}
\def\bOmega{\boldsymbol{\Omega}}

% Mathbf lower case English alphabets
\def\mba{\mathbf{a}}
\def\mbb{\mathbf{b}}
\def\mbc{\mathbf{c}}
\def\mbd{\mathbf{d}}
\def\mbe{\mathbf{e}}
\def\mbf{\mathbf{f}}
\def\mbg{\mathbf{g}}
\def\mbh{\mathbf{h}}
\def\mbi{\mathbf{i}}
\def\mbj{\mathbf{j}}
\def\mbk{\mathbf{k}}
\def\mbl{\mathbf{l}}
\def\mbm{\mathbf{m}}
\def\mbn{\mathbf{n}}
\def\mbo{\mathbf{o}}
\def\mbp{\mathbf{p}}
\def\mbq{\mathbf{q}}
\def\mbr{\mathbf{r}}
\def\mbs{\mathbf{s}}
\def\mbt{\mathbf{t}}
\def\mbu{\mathbf{u}}
\def\mbv{\mathbf{v}}
\def\mbw{\mathbf{w}}
\def\mbx{\mathbf{x}}
\def\mby{\mathbf{y}}
\def\mbz{\mathbf{z}}

% Mathbf upper case English alphabets
\def\mbA{\mathbf{A}}
\def\mbB{\mathbf{B}}
\def\mbC{\mathbf{C}}
\def\mbD{\mathbf{D}}
\def\mbE{\mathbf{E}}
\def\mbF{\mathbf{F}}
\def\mbG{\mathbf{G}}
\def\mbH{\mathbf{H}}
\def\mbI{\mathbf{I}}
\def\mbJ{\mathbf{J}}
\def\mbK{\mathbf{K}}
\def\mbL{\mathbf{L}}
\def\mbM{\mathbf{M}}
\def\mbN{\mathbf{N}}
\def\mbO{\mathbf{O}}
\def\mbP{\mathbf{P}}
\def\mbQ{\mathbf{Q}}
\def\mbR{\mathbf{R}}
\def\mbS{\mathbf{S}}
\def\mbT{\mathbf{T}}
\def\mbU{\mathbf{U}}
\def\mbV{\mathbf{V}}
\def\mbW{\mathbf{W}}
\def\mbX{\mathbf{X}}
\def\mbY{\mathbf{Y}}
\def\mbZ{\mathbf{Z}}

% Caligraphy upper case English alphabets
\def\calA{\mathcal{A}}
\def\calB{\mathcal{B}}
\def\calC{\mathcal{C}}
\def\calD{\mathcal{D}}
\def\calE{\mathcal{E}}
\def\calF{\mathcal{F}}
\def\calG{\mathcal{G}}
\def\calH{\mathcal{H}}
\def\calI{\mathcal{I}}
\def\calJ{\mathcal{J}}
\def\calK{\mathcal{K}}
\def\calL{\mathcal{L}}
\def\calM{\mathcal{M}}
\def\calN{\mathcal{N}}
\def\calO{\mathcal{O}}
\def\calP{\mathcal{P}}
\def\calQ{\mathcal{Q}}
\def\calR{\mathcal{R}}
\def\calS{\mathcal{S}}
\def\calT{\mathcal{T}}
\def\calU{\mathcal{U}}
\def\calV{\mathcal{V}}
\def\calW{\mathcal{W}}
\def\calX{\mathcal{X}}
\def\calY{\mathcal{Y}}
\def\calZ{\mathcal{Z}}

% Numbers
\def\bzero{\boldsymbol{0}}
\def\bone{\boldsymbol{1}}

% Sets and notations
\newcommand{\binaryB}[1]{\mathds{B}^{#1}}
\newcommand{\complexC}[1]{\mathds{C}^{#1}}
\newcommand{\expecE}[1]{\mathds{E}\left\{{#1}\right\}}
\newcommand{\naturalN}[1]{\mathds{N}^{#1}}
\newcommand{\probP}[1]{\mathds{P}\mathrm{r}\left\{{#1}\right\}}
\newcommand{\rationalQ}[1]{\mathds{Q}^{#1}}
\newcommand{\realR}[1]{\mathds{R}^{#1}}
\newcommand{\realRp}[1]{\mathds{R}_{+}^{#1}}
\newcommand{\realRn}[1]{\mathds{R}_{-}^{#1}}
\newcommand{\integerZ}[1]{\mathds{Z}^{#1}}

% Matrix terms
\def\Tr#1{\mathrm{Tr}\left(#1\right)}
\def\vec#1{\mathrm{vec}\left(#1\right)}
\def\diag#1{\mathrm{diag}\left(#1\right)}
\def\Diag#1{\mathrm{Diag}\left(#1\right)}
\def\bdiag#1{\mathbf{diag}\left(#1\right)}
\def\cov#1{\mathrm{cov}\left(#1\right)}
\def\Cov#1{\mathrm{Cov}\left(#1\right)}
\def\bcov#1{\mathbf{cov}\left(#1\right)}

% Misc
\def\asin#1{\sin^{-1}\left(#1\right)}
\def\acos#1{\cos^{-1}\left(#1\right)}
\def\atan#1{\tan^{-1}\left(#1\right)}
\def\acsc#1{\csc^{-1}\left(#1\right)}
\def\asec#1{\sec^{-1}\left(#1\right)}
\def\acot#1{\cot^{-1}\left(#1\right)}
\def\implies{\Rightarrow}
\def\half{\frac{1}{2}}
\def\roothalf{\frac{1}{\sqrt{2}}}
\def\third{\frac{1}{3}}
\def\quarter{\frac{1}{4}}
\def\fourth{\frac{1}{4}}
\def\fifth{\frac{1}{5}}
\def\threequarter{\frac{3}{4}}
\def\ejomg{e^{j\omega}}
\def\ejnomg{e^{-j\omega}}
\def\zinv{z^{-1}}
\def\sgn#1{\mathrm{sgn}\left(#1\right)}
\def\sign#1{\mathrm{sign}\left(#1\right)}
\def\csign#1{\mathrm{csign}\left(#1\right)}
\def\deg{^\circ}
\def\Oh#1{\mathcal{O}\left(#1\right)}
\def\oh#1{o\left(#1\right)}
\def\d#1{\mathrm{d}#1}
\def\st{~\mathrm{s.t.}~}
\def\ow{~\mathrm{otherwise}~}
\def\ew{~\mathrm{elsewhere}~}
\def\eg{\emph{e.g.}}
\def\ie{\emph{i.e.}}
\def\etal{\emph{et al.}}
\def\etc{\emph{etc.}}
\def\viz{\emph{viz.}}
\def\conv{\circledast}
\def\Re#1{\operatorname{Re}\left(#1\right)}
\def\Im#1{\operatorname{Im}\left(#1\right)}
\def\arg#1{\operatorname{arg}\left(#1\right)}

% Basic text colors
\def\white#1{\textcolor{white}{#1}}
\def\black#1{\textcolor{black}{#1}}
\def\red#1{\textcolor{red}{#1}}
\def\green#1{\textcolor{green}{#1}}
\def\blue#1{\textcolor{blue}{#1}}
\def\cyan#1{\textcolor{cyan}{#1}}
\def\magenta#1{\textcolor{magenta}{#1}}
\def\yellow#1{\textcolor{yellow}{#1}}

% Special colors that comes with [dvipsnames] option in xcolor package
\def\Apricot#1{\textcolor{Apricot}{#1}}
\def\Aquamarine#1{\textcolor{Aquamarine}{#1}}
\def\Bittersweet#1{\textcolor{Bittersweet}{#1}}
\def\Black#1{\textcolor{Black}{#1}}
\def\Blue#1{\textcolor{Blue}{#1}}
\def\BlueGreen#1{\textcolor{BlueGreen}{#1}}
\def\BlueViolet#1{\textcolor{BlueViolet}{#1}}
\def\BrickRed#1{\textcolor{BrickRed}{#1}}
\def\Brown#1{\textcolor{Brown}{#1}}
\def\BurntOrange#1{\textcolor{BurntOrange}{#1}}
\def\CadetBlue#1{\textcolor{CadetBlue}{#1}}
\def\CarnationPink#1{\textcolor{CarnationPink}{#1}}
\def\Cerulean#1{\textcolor{Cerulean}{#1}}
\def\CornflowerBlue#1{\textcolor{CornflowerBlue}{#1}}
\def\Cyan#1{\textcolor{Cyan}{#1}}
\def\Dandelion#1{\textcolor{Dandelion}{#1}}
\def\DarkOrchid#1{\textcolor{DarkOrchid}{#1}}
\def\Emerald#1{\textcolor{Emerald}{#1}}
\def\ForestGreen#1{\textcolor{ForestGreen}{#1}}
\def\Fuchsia#1{\textcolor{Fuchsia}{#1}}
\def\Goldenrod#1{\textcolor{Goldenrod}{#1}}
\def\Gray#1{\textcolor{Gray}{#1}}
\def\Green#1{\textcolor{Green}{#1}}
\def\GreenYellow#1{\textcolor{GreenYellow}{#1}}
\def\JungleGreen#1{\textcolor{JungleGreen}{#1}}
\def\Lavender#1{\textcolor{Lavender}{#1}}
\def\LimeGreen#1{\textcolor{LimeGreen}{#1}}
\def\Magenta#1{\textcolor{Magenta}{#1}}
\def\Mahogany#1{\textcolor{Mahogany}{#1}}
\def\Maroon#1{\textcolor{Maroon}{#1}}
\def\Melon#1{\textcolor{Melon}{#1}}
\def\MidnightBlue#1{\textcolor{MidnightBlue}{#1}}
\def\Mulberry#1{\textcolor{Mulberry}{#1}}
\def\NavyBlue#1{\textcolor{NavyBlue}{#1}}
\def\OliveGreen#1{\textcolor{OliveGreen}{#1}}
\def\Orange#1{\textcolor{Orange}{#1}}
\def\OrangeRed#1{\textcolor{OrangeRed}{#1}}
\def\Orchid#1{\textcolor{Orchid}{#1}}
\def\Peach#1{\textcolor{Peach}{#1}}
\def\Periwinkle#1{\textcolor{Periwinkle}{#1}}
\def\PineGreen#1{\textcolor{PineGreen}{#1}}
\def\Plum#1{\textcolor{Plum}{#1}}
\def\ProcessBlue#1{\textcolor{ProcessBlue}{#1}}
\def\Purple#1{\textcolor{Purple}{#1}}
\def\RawSienna#1{\textcolor{RawSienna}{#1}}
\def\Red#1{\textcolor{Red}{#1}}
\def\RedOrange#1{\textcolor{RedOrange}{#1}}
\def\RedViolet#1{\textcolor{RedViolet}{#1}}
\def\Rhodamine#1{\textcolor{Rhodamine}{#1}}
\def\RoyalBlue#1{\textcolor{RoyalBlue}{#1}}
\def\RoyalPurple#1{\textcolor{RoyalPurple}{#1}}
\def\RubineRed#1{\textcolor{RubineRed}{#1}}
\def\Salmon#1{\textcolor{Salmon}{#1}}
\def\SeaGreen#1{\textcolor{SeaGreen}{#1}}
\def\Sepia#1{\textcolor{Sepia}{#1}}
\def\YellowOrange#1{\textcolor{YellowOrange}{#1}}
\def\SkyBlue#1{\textcolor{SkyBlue}{#1}}
\def\SpringGreen#1{\textcolor{SpringGreen}{#1}}
\def\Tan#1{\textcolor{Tan}{#1}}
\def\TealBlue#1{\textcolor{TealBlue}{#1}}
\def\Thistle#1{\textcolor{Thistle}{#1}}
\def\Turquoise#1{\textcolor{Turquoise}{#1}}
\def\Violet#1{\textcolor{Violet}{#1}}
\def\VioletRed#1{\textcolor{VioletRed}{#1}}
\def\White#1{\textcolor{White}{#1}}
\def\WildStrawberry#1{\textcolor{WildStrawberry}{#1}}
\def\Yellow#1{\textcolor{Yellow}{#1}}
\def\YellowGreen#1{\textcolor{YellowGreen}{#1}}
\def\YellowOrange#1{\textcolor{YellowOrange}{#1}}

% Theorem-like environments (defs, lemmas numbered like Theorems)
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{example}{Example}
%\theoremstyle{definition}
\newtheorem{definition}{Definition}
%\theoremstyle{remark}
\newtheorem{remark}{Remark}

%\declaretheorem[style=definition,name=Remark,qed=$\blacksquare$]{remark}

% algorithms
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Initialize:}}
%\algnewcommand\algorithmicinput{\textbf{Input:}}
%\algnewcommand\Input{\item[\algorithmicinput]}
%\algnewcommand\algorithmicoutput{\textbf{Output:}}
%\algnewcommand\Output{\item[\algorithmicoutput]}
%\algnewcommand\algorithmicinit{\textbf{Initialize:}}
%\algnewcommand\Init{\item[\algorithmicinit]}
\def\Print#1{\textbf{print}~#1}
\def\To{\textbf{to}~}

% underbrace inside a matrix environment
\newcommand\undermat[2]{
	\makebox[0pt][l]{${\underbrace{\hphantom{
					\begin{matrix}#1\end{matrix}}}_{\text{$#2$}}}$}#1}
					
					
\def\LoS{{\textrm{LoS}}}
\def\NLoS{{\textrm{NLoS}}}
\def\PRI{{\textrm{PRI}}}
\def\T{\top}
\def\H{\mathrm{H}}
\def\j{\mathrm{j}}
\def\vecinv#1{\mathrm{vec}^{-1}\left(#1\right)}






==> ICASSP 2023_ Joint Waveform and Beamforming Design in Multi-IRS Aided Radar/symbols_1.tex <==
%% Short symbol commands for LaTex
\usepackage{amsmath}
\usepackage{algpseudocode}
\usepackage{amsthm}
\usepackage{dsfont}
%\usepackage[lined,boxed,commentsnumbered]{algorithm2e}
\usepackage{algorithm}
\usepackage{thmtools}
\usepackage{amssymb}
\usepackage[dvipsnames]{xcolor}


\def \Version{2.0.10}
\def \Update{\today}

% Lower case bold English alphabets
\def\ba{\boldsymbol{a}}
\def\bb{\boldsymbol{b}}
\def\bc{\boldsymbol{c}}
\def\bd{\boldsymbol{d}}
\def\be{\boldsymbol{e}}
\def\bdf{\boldsymbol{f}}
\def\bg{\boldsymbol{g}}
\def\bh{\boldsymbol{h}}
\def\bi{\boldsymbol{i}}
\def\bj{\boldsymbol{j}}
\def\bk{\boldsymbol{k}}
\def\bl{\boldsymbol{l}}
\def\bm{\boldsymbol{m}}
\def\bn{\boldsymbol{n}}
\def\bo{\boldsymbol{o}}
\def\bp{\boldsymbol{p}}
\def\bq{\boldsymbol{q}}
\def\br{\boldsymbol{r}}
\def\bs{\boldsymbol{s}}
\def\bt{\boldsymbol{t}}
\def\bu{\boldsymbol{u}}
\def\bv{\boldsymbol{v}}
\def\bw{\boldsymbol{w}}
\def\bx{\boldsymbol{x}}
\def\by{\boldsymbol{y}}
\def\bz{\boldsymbol{z}}

% Upper case bold English alphabets
\def\bA{\boldsymbol{A}}
\def\bB{\boldsymbol{B}}
\def\bC{\boldsymbol{C}}
\def\bD{\boldsymbol{D}}
\def\bE{\boldsymbol{E}}
\def\bF{\boldsymbol{F}}
\def\bG{\boldsymbol{G}}
\def\bH{\boldsymbol{H}}
\def\bI{\boldsymbol{I}}
\def\bJ{\boldsymbol{J}}
\def\bK{\boldsymbol{K}}
\def\bL{\boldsymbol{L}}
\def\bN{\boldsymbol{N}}
\def\bM{\boldsymbol{M}}
\def\bO{\boldsymbol{O}}
\def\bP{\boldsymbol{P}}
\def\bQ{\boldsymbol{Q}}
\def\bR{\boldsymbol{R}}
\def\bS{\boldsymbol{S}}
\def\bT{\boldsymbol{T}}
\def\bU{\boldsymbol{U}}
\def\bV{\boldsymbol{V}}
\def\bW{\boldsymbol{W}}
\def\bX{\boldsymbol{X}}
\def\bY{\boldsymbol{Y}}
\def\bZ{\boldsymbol{Z}}

% Bold Greek alphabets
\def\balpha{\boldsymbol{\alpha}}
\def\bbeta{\boldsymbol{\beta}}
\def\bgamma{\boldsymbol{\gamma}}
\def\bGamma{\boldsymbol{\Gamma}}
\def\bdelta{\boldsymbol{\delta}}
\def\bDelta{\boldsymbol{\Delta}}
\def\bepsilon{\boldsymbol{\epsilon}}
\def\bvarepsilon{\boldsymbol{\varepsilon}}
\def\bzeta{\boldsymbol{\zeta}}
\def\bdeta{\boldsymbol{\eta}}
\def\btheta{\boldsymbol{\theta}}
\def\bvartheta{\boldsymbol{\vartheta}}
\def\bTheta{\boldsymbol{\Theta}}
\def\biota{\boldsymbol{\iota}}
\def\bkappa{\boldsymbol{\kappa}}
\def\blambda{\boldsymbol{\lambda}}
\def\bLambda{\boldsymbol{\Lambda}}
\def\bmu{\boldsymbol{\mu}}
\def\bnu{\boldsymbol{\nu}}
\def\bxi{\boldsymbol{\xi}}
\def\bXi{\boldsymbol{\Xi}}
\def\bpi{\boldsymbol{\pi}}
\def\bPi{\boldsymbol{\Pi}}
\def\brho{\boldsymbol{\rho}}
\def\bvarrho{\boldsymbol{\varrho}}
\def\bsigma{\boldsymbol{\sigma}}
\def\bSigma{\boldsymbol{\Sigma}}
\def\btau{\boldsymbol{\tau}}
\def\bupsilon{\boldsymbol{\upsilon}}
\def\bUpsilon{\boldsymbol{\Upsilon}}
\def\bphi{\boldsymbol{\phi}}
\def\bvarphi{\boldsymbol{\varphi}}
\def\bPhi{\boldsymbol{\Phi}}
\def\bchi{\boldsymbol{\chi}}
\def\bpsi{\boldsymbol{\psi}}
\def\bPsi{\boldsymbol{\Psi}}
\def\bomega{\boldsymbol{\omega}}
\def\bOmega{\boldsymbol{\Omega}}

% Mathbf lower case English alphabets
\def\mba{\mathbf{a}}
\def\mbb{\mathbf{b}}
\def\mbc{\mathbf{c}}
\def\mbd{\mathbf{d}}
\def\mbe{\mathbf{e}}
\def\mbf{\mathbf{f}}
\def\mbg{\mathbf{g}}
\def\mbh{\mathbf{h}}
\def\mbi{\mathbf{i}}
\def\mbj{\mathbf{j}}
\def\mbk{\mathbf{k}}
\def\mbl{\mathbf{l}}
\def\mbm{\mathbf{m}}
\def\mbn{\mathbf{n}}
\def\mbo{\mathbf{o}}
\def\mbp{\mathbf{p}}
\def\mbq{\mathbf{q}}
\def\mbr{\mathbf{r}}
\def\mbs{\mathbf{s}}
\def\mbt{\mathbf{t}}
\def\mbu{\mathbf{u}}
\def\mbv{\mathbf{v}}
\def\mbw{\mathbf{w}}
\def\mbx{\mathbf{x}}
\def\mby{\mathbf{y}}
\def\mbz{\mathbf{z}}

% Mathbf upper case English alphabets
\def\mbA{\mathbf{A}}
\def\mbB{\mathbf{B}}
\def\mbC{\mathbf{C}}
\def\mbD{\mathbf{D}}
\def\mbE{\mathbf{E}}
\def\mbF{\mathbf{F}}
\def\mbG{\mathbf{G}}
\def\mbH{\mathbf{H}}
\def\mbI{\mathbf{I}}
\def\mbJ{\mathbf{J}}
\def\mbK{\mathbf{K}}
\def\mbL{\mathbf{L}}
\def\mbM{\mathbf{M}}
\def\mbN{\mathbf{N}}
\def\mbO{\mathbf{O}}
\def\mbP{\mathbf{P}}
\def\mbQ{\mathbf{Q}}
\def\mbR{\mathbf{R}}
\def\mbS{\mathbf{S}}
\def\mbT{\mathbf{T}}
\def\mbU{\mathbf{U}}
\def\mbV{\mathbf{V}}
\def\mbW{\mathbf{W}}
\def\mbX{\mathbf{X}}
\def\mbY{\mathbf{Y}}
\def\mbZ{\mathbf{Z}}

% Caligraphy upper case English alphabets
\def\calA{\mathcal{A}}
\def\calB{\mathcal{B}}
\def\calC{\mathcal{C}}
\def\calD{\mathcal{D}}
\def\calE{\mathcal{E}}
\def\calF{\mathcal{F}}
\def\calG{\mathcal{G}}
\def\calH{\mathcal{H}}
\def\calI{\mathcal{I}}
\def\calJ{\mathcal{J}}
\def\calK{\mathcal{K}}
\def\calL{\mathcal{L}}
\def\calM{\mathcal{M}}
\def\calN{\mathcal{N}}
\def\calO{\mathcal{O}}
\def\calP{\mathcal{P}}
\def\calQ{\mathcal{Q}}
\def\calR{\mathcal{R}}
\def\calS{\mathcal{S}}
\def\calT{\mathcal{T}}
\def\calU{\mathcal{U}}
\def\calV{\mathcal{V}}
\def\calW{\mathcal{W}}
\def\calX{\mathcal{X}}
\def\calY{\mathcal{Y}}
\def\calZ{\mathcal{Z}}

% Numbers
\def\bzero{\boldsymbol{0}}
\def\bone{\boldsymbol{1}}

% Sets and notations
\newcommand{\binaryB}[1]{\mathds{B}^{#1}}
\newcommand{\complexC}[1]{\mathds{C}^{#1}}
\newcommand{\expecE}[1]{\mathds{E}\left\{{#1}\right\}}
\newcommand{\naturalN}[1]{\mathds{N}^{#1}}
\newcommand{\probP}[1]{\mathds{P}\mathrm{r}\left\{{#1}\right\}}
\newcommand{\rationalQ}[1]{\mathds{Q}^{#1}}
\newcommand{\realR}[1]{\mathds{R}^{#1}}
\newcommand{\realRp}[1]{\mathds{R}_{+}^{#1}}
\newcommand{\realRn}[1]{\mathds{R}_{-}^{#1}}
\newcommand{\integerZ}[1]{\mathds{Z}^{#1}}

% Matrix terms
\def\tr#1{\mathrm{Tr}\left(#1\right)}
\def\vec#1{\mathrm{vec}\left(#1\right)}
\def\diag#1{\mathrm{diag}\left(#1\right)}
\def\Diag#1{\mathrm{Diag}\left(#1\right)}
\def\bdiag#1{\mathbf{diag}\left(#1\right)}
\def\cov#1{\mathrm{cov}\left(#1\right)}
\def\Cov#1{\mathrm{Cov}\left(#1\right)}
\def\bcov#1{\mathbf{cov}\left(#1\right)}

% Misc
\def\asin#1{\sin^{-1}\left(#1\right)}
\def\acos#1{\cos^{-1}\left(#1\right)}
\def\atan#1{\tan^{-1}\left(#1\right)}
\def\acsc#1{\csc^{-1}\left(#1\right)}
\def\asec#1{\sec^{-1}\left(#1\right)}
\def\acot#1{\cot^{-1}\left(#1\right)}
\def\implies{\Rightarrow}
\def\half{\frac{1}{2}}
\def\roothalf{\frac{1}{\sqrt{2}}}
\def\third{\frac{1}{3}}
\def\quarter{\frac{1}{4}}
\def\fourth{\frac{1}{4}}
\def\fifth{\frac{1}{5}}
\def\threequarter{\frac{3}{4}}
\def\ejomg{e^{j\omega}}
\def\ejnomg{e^{-j\omega}}
\def\zinv{z^{-1}}
\def\sgn#1{\mathrm{sgn}\left(#1\right)}
\def\sign#1{\mathrm{sign}\left(#1\right)}
\def\csign#1{\mathrm{csign}\left(#1\right)}
\def\deg{^\circ}
\def\Oh#1{\mathcal{O}\left(#1\right)}
\def\oh#1{o\left(#1\right)}
\def\d#1{\mathrm{d}#1}
\def\st{~\mathrm{s.t.}~}
\def\ow{~\mathrm{otherwise}~}
\def\ew{~\mathrm{elsewhere}~}
\def\eg{\emph{e.g.}}
\def\ie{\emph{i.e.}}
\def\etal{\emph{et al.}}
\def\etc{\emph{etc.}}
\def\viz{\emph{viz.}}
\def\conv{\circledast}

% Basic text colors
\def\white#1{\textcolor{white}{#1}}
\def\black#1{\textcolor{black}{#1}}
\def\red#1{\textcolor{red}{#1}}
\def\green#1{\textcolor{green}{#1}}
\def\blue#1{\textcolor{blue}{#1}}
\def\cyan#1{\textcolor{cyan}{#1}}
\def\magenta#1{\textcolor{magenta}{#1}}
\def\yellow#1{\textcolor{yellow}{#1}}

% Special colors that comes with [dvipsnames] option in xcolor package
\def\Apricot#1{\textcolor{Apricot}{#1}}
\def\Aquamarine#1{\textcolor{Aquamarine}{#1}}
\def\Bittersweet#1{\textcolor{Bittersweet}{#1}}
\def\Black#1{\textcolor{Black}{#1}}
\def\Blue#1{\textcolor{Blue}{#1}}
\def\BlueGreen#1{\textcolor{BlueGreen}{#1}}
\def\BlueViolet#1{\textcolor{BlueViolet}{#1}}
\def\BrickRed#1{\textcolor{BrickRed}{#1}}
\def\Brown#1{\textcolor{Brown}{#1}}
\def\BurntOrange#1{\textcolor{BurntOrange}{#1}}
\def\CadetBlue#1{\textcolor{CadetBlue}{#1}}
\def\CarnationPink#1{\textcolor{CarnationPink}{#1}}
\def\Cerulean#1{\textcolor{Cerulean}{#1}}
\def\CornflowerBlue#1{\textcolor{CornflowerBlue}{#1}}
\def\Cyan#1{\textcolor{Cyan}{#1}}
\def\Dandelion#1{\textcolor{Dandelion}{#1}}
\def\DarkOrchid#1{\textcolor{DarkOrchid}{#1}}
\def\Emerald#1{\textcolor{Emerald}{#1}}
\def\ForestGreen#1{\textcolor{ForestGreen}{#1}}
\def\Fuchsia#1{\textcolor{Fuchsia}{#1}}
\def\Goldenrod#1{\textcolor{Goldenrod}{#1}}
\def\Gray#1{\textcolor{Gray}{#1}}
\def\Green#1{\textcolor{Green}{#1}}
\def\GreenYellow#1{\textcolor{GreenYellow}{#1}}
\def\JungleGreen#1{\textcolor{JungleGreen}{#1}}
\def\Lavender#1{\textcolor{Lavender}{#1}}
\def\LimeGreen#1{\textcolor{LimeGreen}{#1}}
\def\Magenta#1{\textcolor{Magenta}{#1}}
\def\Mahogany#1{\textcolor{Mahogany}{#1}}
\def\Maroon#1{\textcolor{Maroon}{#1}}
\def\Melon#1{\textcolor{Melon}{#1}}
\def\MidnightBlue#1{\textcolor{MidnightBlue}{#1}}
\def\Mulberry#1{\textcolor{Mulberry}{#1}}
\def\NavyBlue#1{\textcolor{NavyBlue}{#1}}
\def\OliveGreen#1{\textcolor{OliveGreen}{#1}}
\def\Orange#1{\textcolor{Orange}{#1}}
\def\OrangeRed#1{\textcolor{OrangeRed}{#1}}
\def\Orchid#1{\textcolor{Orchid}{#1}}
\def\Peach#1{\textcolor{Peach}{#1}}
\def\Periwinkle#1{\textcolor{Periwinkle}{#1}}
\def\PineGreen#1{\textcolor{PineGreen}{#1}}
\def\Plum#1{\textcolor{Plum}{#1}}
\def\ProcessBlue#1{\textcolor{ProcessBlue}{#1}}
\def\Purple#1{\textcolor{Purple}{#1}}
\def\RawSienna#1{\textcolor{RawSienna}{#1}}
\def\Red#1{\textcolor{Red}{#1}}
\def\RedOrange#1{\textcolor{RedOrange}{#1}}
\def\RedViolet#1{\textcolor{RedViolet}{#1}}
\def\Rhodamine#1{\textcolor{Rhodamine}{#1}}
\def\RoyalBlue#1{\textcolor{RoyalBlue}{#1}}
\def\RoyalPurple#1{\textcolor{RoyalPurple}{#1}}
\def\RubineRed#1{\textcolor{RubineRed}{#1}}
\def\Salmon#1{\textcolor{Salmon}{#1}}
\def\SeaGreen#1{\textcolor{SeaGreen}{#1}}
\def\Sepia#1{\textcolor{Sepia}{#1}}
\def\YellowOrange#1{\textcolor{YellowOrange}{#1}}
\def\SkyBlue#1{\textcolor{SkyBlue}{#1}}
\def\SpringGreen#1{\textcolor{SpringGreen}{#1}}
\def\Tan#1{\textcolor{Tan}{#1}}
\def\TealBlue#1{\textcolor{TealBlue}{#1}}
\def\Thistle#1{\textcolor{Thistle}{#1}}
\def\Turquoise#1{\textcolor{Turquoise}{#1}}
\def\Violet#1{\textcolor{Violet}{#1}}
\def\VioletRed#1{\textcolor{VioletRed}{#1}}
\def\White#1{\textcolor{White}{#1}}
\def\WildStrawberry#1{\textcolor{WildStrawberry}{#1}}
\def\Yellow#1{\textcolor{Yellow}{#1}}
\def\YellowGreen#1{\textcolor{YellowGreen}{#1}}
\def\YellowOrange#1{\textcolor{YellowOrange}{#1}}

% Theorem-like environments (defs, lemmas numbered like Theorems)
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{example}{Example}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\declaretheorem[style=definition,name=Remark,qed=$\blacksquare$]{remark}

% algorithms
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Initialize:}}
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}
\algnewcommand\algorithmicoutput{\textbf{Output:}}
\algnewcommand\Output{\item[\algorithmicoutput]}
\algnewcommand\algorithmicinit{\textbf{Initialize:}}
\algnewcommand\Init{\item[\algorithmicinit]}
\def\Print#1{\textbf{print}~#1}
\def\To{\textbf{to}~}

% underbrace inside a matrix environment
\newcommand\undermat[2]{
	\makebox[0pt][l]{${\underbrace{\hphantom{
					\begin{matrix}#1\end{matrix}}}_{\text{$#2$}}}$}#1}

==> symbols_1.tex <==
%% Short symbol commands for LaTex
\usepackage{amsmath}
\usepackage{algpseudocode}
\usepackage{amsthm}
\usepackage{dsfont}
%\usepackage[lined,boxed,commentsnumbered]{algorithm2e}
\usepackage{algorithm}
\usepackage{thmtools}
\usepackage{amssymb}
\usepackage[dvipsnames]{xcolor}


\def \Version{2.0.10}
\def \Update{\today}

% Lower case bold English alphabets
\def\ba{\boldsymbol{a}}
\def\bb{\boldsymbol{b}}
\def\bc{\boldsymbol{c}}
\def\bd{\boldsymbol{d}}
\def\be{\boldsymbol{e}}
\def\bdf{\boldsymbol{f}}
\def\bg{\boldsymbol{g}}
\def\bh{\boldsymbol{h}}
\def\bi{\boldsymbol{i}}
\def\bj{\boldsymbol{j}}
\def\bk{\boldsymbol{k}}
\def\bl{\boldsymbol{l}}
\def\bm{\boldsymbol{m}}
\def\bn{\boldsymbol{n}}
\def\bo{\boldsymbol{o}}
\def\bp{\boldsymbol{p}}
\def\bq{\boldsymbol{q}}
\def\br{\boldsymbol{r}}
\def\bs{\boldsymbol{s}}
\def\bt{\boldsymbol{t}}
\def\bu{\boldsymbol{u}}
\def\bv{\boldsymbol{v}}
\def\bw{\boldsymbol{w}}
\def\bx{\boldsymbol{x}}
\def\by{\boldsymbol{y}}
\def\bz{\boldsymbol{z}}

% Upper case bold English alphabets
\def\bA{\boldsymbol{A}}
\def\bB{\boldsymbol{B}}
\def\bC{\boldsymbol{C}}
\def\bD{\boldsymbol{D}}
\def\bE{\boldsymbol{E}}
\def\bF{\boldsymbol{F}}
\def\bG{\boldsymbol{G}}
\def\bH{\boldsymbol{H}}
\def\bI{\boldsymbol{I}}
\def\bJ{\boldsymbol{J}}
\def\bK{\boldsymbol{K}}
\def\bL{\boldsymbol{L}}
\def\bN{\boldsymbol{N}}
\def\bM{\boldsymbol{M}}
\def\bO{\boldsymbol{O}}
\def\bP{\boldsymbol{P}}
\def\bQ{\boldsymbol{Q}}
\def\bR{\boldsymbol{R}}
\def\bS{\boldsymbol{S}}
\def\bT{\boldsymbol{T}}
\def\bU{\boldsymbol{U}}
\def\bV{\boldsymbol{V}}
\def\bW{\boldsymbol{W}}
\def\bX{\boldsymbol{X}}
\def\bY{\boldsymbol{Y}}
\def\bZ{\boldsymbol{Z}}

% Bold Greek alphabets
\def\balpha{\boldsymbol{\alpha}}
\def\bbeta{\boldsymbol{\beta}}
\def\bgamma{\boldsymbol{\gamma}}
\def\bGamma{\boldsymbol{\Gamma}}
\def\bdelta{\boldsymbol{\delta}}
\def\bDelta{\boldsymbol{\Delta}}
\def\bepsilon{\boldsymbol{\epsilon}}
\def\bvarepsilon{\boldsymbol{\varepsilon}}
\def\bzeta{\boldsymbol{\zeta}}
\def\bdeta{\boldsymbol{\eta}}
\def\btheta{\boldsymbol{\theta}}
\def\bvartheta{\boldsymbol{\vartheta}}
\def\bTheta{\boldsymbol{\Theta}}
\def\biota{\boldsymbol{\iota}}
\def\bkappa{\boldsymbol{\kappa}}
\def\blambda{\boldsymbol{\lambda}}
\def\bLambda{\boldsymbol{\Lambda}}
\def\bmu{\boldsymbol{\mu}}
\def\bnu{\boldsymbol{\nu}}
\def\bxi{\boldsymbol{\xi}}
\def\bXi{\boldsymbol{\Xi}}
\def\bpi{\boldsymbol{\pi}}
\def\bPi{\boldsymbol{\Pi}}
\def\brho{\boldsymbol{\rho}}
\def\bvarrho{\boldsymbol{\varrho}}
\def\bsigma{\boldsymbol{\sigma}}
\def\bSigma{\boldsymbol{\Sigma}}
\def\btau{\boldsymbol{\tau}}
\def\bupsilon{\boldsymbol{\upsilon}}
\def\bUpsilon{\boldsymbol{\Upsilon}}
\def\bphi{\boldsymbol{\phi}}
\def\bvarphi{\boldsymbol{\varphi}}
\def\bPhi{\boldsymbol{\Phi}}
\def\bchi{\boldsymbol{\chi}}
\def\bpsi{\boldsymbol{\psi}}
\def\bPsi{\boldsymbol{\Psi}}
\def\bomega{\boldsymbol{\omega}}
\def\bOmega{\boldsymbol{\Omega}}

% Mathbf lower case English alphabets
\def\mba{\mathbf{a}}
\def\mbb{\mathbf{b}}
\def\mbc{\mathbf{c}}
\def\mbd{\mathbf{d}}
\def\mbe{\mathbf{e}}
\def\mbf{\mathbf{f}}
\def\mbg{\mathbf{g}}
\def\mbh{\mathbf{h}}
\def\mbi{\mathbf{i}}
\def\mbj{\mathbf{j}}
\def\mbk{\mathbf{k}}
\def\mbl{\mathbf{l}}
\def\mbm{\mathbf{m}}
\def\mbn{\mathbf{n}}
\def\mbo{\mathbf{o}}
\def\mbp{\mathbf{p}}
\def\mbq{\mathbf{q}}
\def\mbr{\mathbf{r}}
\def\mbs{\mathbf{s}}
\def\mbt{\mathbf{t}}
\def\mbu{\mathbf{u}}
\def\mbv{\mathbf{v}}
\def\mbw{\mathbf{w}}
\def\mbx{\mathbf{x}}
\def\mby{\mathbf{y}}
\def\mbz{\mathbf{z}}

% Mathbf upper case English alphabets
\def\mbA{\mathbf{A}}
\def\mbB{\mathbf{B}}
\def\mbC{\mathbf{C}}
\def\mbD{\mathbf{D}}
\def\mbE{\mathbf{E}}
\def\mbF{\mathbf{F}}
\def\mbG{\mathbf{G}}
\def\mbH{\mathbf{H}}
\def\mbI{\mathbf{I}}
\def\mbJ{\mathbf{J}}
\def\mbK{\mathbf{K}}
\def\mbL{\mathbf{L}}
\def\mbM{\mathbf{M}}
\def\mbN{\mathbf{N}}
\def\mbO{\mathbf{O}}
\def\mbP{\mathbf{P}}
\def\mbQ{\mathbf{Q}}
\def\mbR{\mathbf{R}}
\def\mbS{\mathbf{S}}
\def\mbT{\mathbf{T}}
\def\mbU{\mathbf{U}}
\def\mbV{\mathbf{V}}
\def\mbW{\mathbf{W}}
\def\mbX{\mathbf{X}}
\def\mbY{\mathbf{Y}}
\def\mbZ{\mathbf{Z}}

% Caligraphy upper case English alphabets
\def\calA{\mathcal{A}}
\def\calB{\mathcal{B}}
\def\calC{\mathcal{C}}
\def\calD{\mathcal{D}}
\def\calE{\mathcal{E}}
\def\calF{\mathcal{F}}
\def\calG{\mathcal{G}}
\def\calH{\mathcal{H}}
\def\calI{\mathcal{I}}
\def\calJ{\mathcal{J}}
\def\calK{\mathcal{K}}
\def\calL{\mathcal{L}}
\def\calM{\mathcal{M}}
\def\calN{\mathcal{N}}
\def\calO{\mathcal{O}}
\def\calP{\mathcal{P}}
\def\calQ{\mathcal{Q}}
\def\calR{\mathcal{R}}
\def\calS{\mathcal{S}}
\def\calT{\mathcal{T}}
\def\calU{\mathcal{U}}
\def\calV{\mathcal{V}}
\def\calW{\mathcal{W}}
\def\calX{\mathcal{X}}
\def\calY{\mathcal{Y}}
\def\calZ{\mathcal{Z}}

% Numbers
\def\bzero{\boldsymbol{0}}
\def\bone{\boldsymbol{1}}

% Sets and notations
\newcommand{\binaryB}[1]{\mathds{B}^{#1}}
\newcommand{\complexC}[1]{\mathds{C}^{#1}}
\newcommand{\expecE}[1]{\mathds{E}\left\{{#1}\right\}}
\newcommand{\naturalN}[1]{\mathds{N}^{#1}}
\newcommand{\probP}[1]{\mathds{P}\mathrm{r}\left\{{#1}\right\}}
\newcommand{\rationalQ}[1]{\mathds{Q}^{#1}}
\newcommand{\realR}[1]{\mathds{R}^{#1}}
\newcommand{\realRp}[1]{\mathds{R}_{+}^{#1}}
\newcommand{\realRn}[1]{\mathds{R}_{-}^{#1}}
\newcommand{\integerZ}[1]{\mathds{Z}^{#1}}

% Matrix terms
\def\tr#1{\mathrm{Tr}\left(#1\right)}
\def\vec#1{\mathrm{vec}\left(#1\right)}
\def\diag#1{\mathrm{diag}\left(#1\right)}
\def\Diag#1{\mathrm{Diag}\left(#1\right)}
\def\bdiag#1{\mathbf{diag}\left(#1\right)}
\def\cov#1{\mathrm{cov}\left(#1\right)}
\def\Cov#1{\mathrm{Cov}\left(#1\right)}
\def\bcov#1{\mathbf{cov}\left(#1\right)}

% Misc
\def\asin#1{\sin^{-1}\left(#1\right)}
\def\acos#1{\cos^{-1}\left(#1\right)}
\def\atan#1{\tan^{-1}\left(#1\right)}
\def\acsc#1{\csc^{-1}\left(#1\right)}
\def\asec#1{\sec^{-1}\left(#1\right)}
\def\acot#1{\cot^{-1}\left(#1\right)}
\def\implies{\Rightarrow}
\def\half{\frac{1}{2}}
\def\roothalf{\frac{1}{\sqrt{2}}}
\def\third{\frac{1}{3}}
\def\quarter{\frac{1}{4}}
\def\fourth{\frac{1}{4}}
\def\fifth{\frac{1}{5}}
\def\threequarter{\frac{3}{4}}
\def\ejomg{e^{j\omega}}
\def\ejnomg{e^{-j\omega}}
\def\zinv{z^{-1}}
\def\sgn#1{\mathrm{sgn}\left(#1\right)}
\def\sign#1{\mathrm{sign}\left(#1\right)}
\def\csign#1{\mathrm{csign}\left(#1\right)}
\def\deg{^\circ}
\def\Oh#1{\mathcal{O}\left(#1\right)}
\def\oh#1{o\left(#1\right)}
\def\d#1{\mathrm{d}#1}
\def\st{~\mathrm{s.t.}~}
\def\ow{~\mathrm{otherwise}~}
\def\ew{~\mathrm{elsewhere}~}
\def\eg{\emph{e.g.}}
\def\ie{\emph{i.e.}}
\def\etal{\emph{et al.}}
\def\etc{\emph{etc.}}
\def\viz{\emph{viz.}}
\def\conv{\circledast}

% Basic text colors
\def\white#1{\textcolor{white}{#1}}
\def\black#1{\textcolor{black}{#1}}
\def\red#1{\textcolor{red}{#1}}
\def\green#1{\textcolor{green}{#1}}
\def\blue#1{\textcolor{blue}{#1}}
\def\cyan#1{\textcolor{cyan}{#1}}
\def\magenta#1{\textcolor{magenta}{#1}}
\def\yellow#1{\textcolor{yellow}{#1}}

% Special colors that comes with [dvipsnames] option in xcolor package
\def\Apricot#1{\textcolor{Apricot}{#1}}
\def\Aquamarine#1{\textcolor{Aquamarine}{#1}}
\def\Bittersweet#1{\textcolor{Bittersweet}{#1}}
\def\Black#1{\textcolor{Black}{#1}}
\def\Blue#1{\textcolor{Blue}{#1}}
\def\BlueGreen#1{\textcolor{BlueGreen}{#1}}
\def\BlueViolet#1{\textcolor{BlueViolet}{#1}}
\def\BrickRed#1{\textcolor{BrickRed}{#1}}
\def\Brown#1{\textcolor{Brown}{#1}}
\def\BurntOrange#1{\textcolor{BurntOrange}{#1}}
\def\CadetBlue#1{\textcolor{CadetBlue}{#1}}
\def\CarnationPink#1{\textcolor{CarnationPink}{#1}}
\def\Cerulean#1{\textcolor{Cerulean}{#1}}
\def\CornflowerBlue#1{\textcolor{CornflowerBlue}{#1}}
\def\Cyan#1{\textcolor{Cyan}{#1}}
\def\Dandelion#1{\textcolor{Dandelion}{#1}}
\def\DarkOrchid#1{\textcolor{DarkOrchid}{#1}}
\def\Emerald#1{\textcolor{Emerald}{#1}}
\def\ForestGreen#1{\textcolor{ForestGreen}{#1}}
\def\Fuchsia#1{\textcolor{Fuchsia}{#1}}
\def\Goldenrod#1{\textcolor{Goldenrod}{#1}}
\def\Gray#1{\textcolor{Gray}{#1}}
\def\Green#1{\textcolor{Green}{#1}}
\def\GreenYellow#1{\textcolor{GreenYellow}{#1}}
\def\JungleGreen#1{\textcolor{JungleGreen}{#1}}
\def\Lavender#1{\textcolor{Lavender}{#1}}
\def\LimeGreen#1{\textcolor{LimeGreen}{#1}}
\def\Magenta#1{\textcolor{Magenta}{#1}}
\def\Mahogany#1{\textcolor{Mahogany}{#1}}
\def\Maroon#1{\textcolor{Maroon}{#1}}
\def\Melon#1{\textcolor{Melon}{#1}}
\def\MidnightBlue#1{\textcolor{MidnightBlue}{#1}}
\def\Mulberry#1{\textcolor{Mulberry}{#1}}
\def\NavyBlue#1{\textcolor{NavyBlue}{#1}}
\def\OliveGreen#1{\textcolor{OliveGreen}{#1}}
\def\Orange#1{\textcolor{Orange}{#1}}
\def\OrangeRed#1{\textcolor{OrangeRed}{#1}}
\def\Orchid#1{\textcolor{Orchid}{#1}}
\def\Peach#1{\textcolor{Peach}{#1}}
\def\Periwinkle#1{\textcolor{Periwinkle}{#1}}
\def\PineGreen#1{\textcolor{PineGreen}{#1}}
\def\Plum#1{\textcolor{Plum}{#1}}
\def\ProcessBlue#1{\textcolor{ProcessBlue}{#1}}
\def\Purple#1{\textcolor{Purple}{#1}}
\def\RawSienna#1{\textcolor{RawSienna}{#1}}
\def\Red#1{\textcolor{Red}{#1}}
\def\RedOrange#1{\textcolor{RedOrange}{#1}}
\def\RedViolet#1{\textcolor{RedViolet}{#1}}
\def\Rhodamine#1{\textcolor{Rhodamine}{#1}}
\def\RoyalBlue#1{\textcolor{RoyalBlue}{#1}}
\def\RoyalPurple#1{\textcolor{RoyalPurple}{#1}}
\def\RubineRed#1{\textcolor{RubineRed}{#1}}
\def\Salmon#1{\textcolor{Salmon}{#1}}
\def\SeaGreen#1{\textcolor{SeaGreen}{#1}}
\def\Sepia#1{\textcolor{Sepia}{#1}}
\def\YellowOrange#1{\textcolor{YellowOrange}{#1}}
\def\SkyBlue#1{\textcolor{SkyBlue}{#1}}
\def\SpringGreen#1{\textcolor{SpringGreen}{#1}}
\def\Tan#1{\textcolor{Tan}{#1}}
\def\TealBlue#1{\textcolor{TealBlue}{#1}}
\def\Thistle#1{\textcolor{Thistle}{#1}}
\def\Turquoise#1{\textcolor{Turquoise}{#1}}
\def\Violet#1{\textcolor{Violet}{#1}}
\def\VioletRed#1{\textcolor{VioletRed}{#1}}
\def\White#1{\textcolor{White}{#1}}
\def\WildStrawberry#1{\textcolor{WildStrawberry}{#1}}
\def\Yellow#1{\textcolor{Yellow}{#1}}
\def\YellowGreen#1{\textcolor{YellowGreen}{#1}}
\def\YellowOrange#1{\textcolor{YellowOrange}{#1}}

% Theorem-like environments (defs, lemmas numbered like Theorems)
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{example}{Example}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\declaretheorem[style=definition,name=Remark,qed=$\blacksquare$]{remark}

% algorithms
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Initialize:}}
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}
\algnewcommand\algorithmicoutput{\textbf{Output:}}
\algnewcommand\Output{\item[\algorithmicoutput]}
\algnewcommand\algorithmicinit{\textbf{Initialize:}}
\algnewcommand\Init{\item[\algorithmicinit]}
\def\Print#1{\textbf{print}~#1}
\def\To{\textbf{to}~}

% underbrace inside a matrix environment
\newcommand\undermat[2]{
	\makebox[0pt][l]{${\underbrace{\hphantom{
					\begin{matrix}#1\end{matrix}}}_{\text{$#2$}}}$}#1}
